Magnet: Multi-turn Tool-use Data Synthesis and Distillation via Graph Translation

Large language models (LLMs) have exhibited the ability to effectively utilize external tools to address user queries. However, their performance may be limited in complex, multi-turn interactions involving users and multiple tools. To address this, we propose Magnet, a principled framework for synthesizing high-quality training trajectories to enhance the function calling capability of large language model agents in multi-turn conversations with humans. The framework is based on automatic and iterative translations from a function signature path to a sequence of queries and executable function calls. We model the complicated function interactions in multi-turn cases with graph and design novel node operations to build reliable signature paths. Motivated by context distillation, when guiding the generation of positive and negative trajectories using a teacher model, we provide reference function call sequences as positive hints in context and contrastive, incorrect function calls as negative hints. Experiments show that training with the positive trajectories with supervised fine-tuning and preference optimization against negative trajectories, our 14B model, Magnet-14B-mDPO, obtains 68.01 on BFCL-v3 and 73.30 on ToolQuery, surpassing the performance of the teacher model Gemini-1.5-pro-002 by a large margin in function calling.

==> tables/qualitative_study.tex <==
\begin{table*}[t]
\definecolor{lightgray}{gray}{0.9}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{|p{1.0\linewidth}|} \hline
\rowcolor{lightgray}
\small \textbf{Example 1 (nested and implicit FC)}: I'm planning a journey from Los Angeles to New York on the morning of April 15th 2024, preferring to fly business class. Arrange this flight using my pre-linked credit card with id 'card\_123456789' and access token 'abc123xyz' \\ 
\hline
\footnotesize Mistake 1 (Not calling necessary functions and hallucinating arguments): \\ \scriptsize \textsc{book\_flight(access\_token='abc123xyz', card\_id='card\_123456789', \dots , travel\_class='business', travel\_cost=\textcolor{red}{1000.0})} \\
\footnotesize Mistake 2 (Composing all functions together but not waiting for tool responses): \\ \scriptsize \textsc{get\_flight\_cost(travel\_from='LAX',travel\_to='JFK',travel\_date='2024-04-15',trave\_class='business'), book\_flight(access\_token='abc123xyz', card\_id='card\_123456789', \dots , travel\_cost=\textcolor{red}{1100.0})} \\
\footnotesize Mistake 3 (Asking for information when actually obtainable): \\ \scriptsize
I need the cost of the flight to help book the flight. Please provide the cost of your flight from Los Angeles to New York.\\ \hline
\footnotesize step 0: [get\_flight\_cost(travel\_from='LAX',travel\_to='JFK',travel\_date='2024-04-15',trave\_class='business')] \\
\bottomrule
% Use Case Navn:& \multicolumn{2}{}{Opret Server} \\ \hline\hline
% Scenarie:& \multicolumn{2}{p{4cm}|}{\raggedright At oprette en server med bestemte regler som tillader folk at spille sammen. More Text more text More Text} \\ \hline
\end{tabular}

% [book_flight(access_token='abc123xyz', card_id='card_123456789', travel_date='2024-04-15', travel_from='LAX', travel_to='JFK', travel_class='business', travel_cost=1000.0)]

% {"role": "tool", "content": "{\"travel_cost_list\": [2400.0]}"}]
% [book_flight(access_token='abc123xyz',card_id='card_123456789',travel_date='2024-04-15',travel_from='LAX',travel_to='JFK',travel_class='business',travel_cost=2400.0)]
% Your flight from LAX to JFK on April 15, 2024 has been booked. Your booking ID is 3426812 and the transaction ID is 45451592.
\vspace{-6pt}
\caption{Example of triplets.}
\label{table:examplesoftriplet}
\end{table*}


% \begin{figure*}[t]
% \small
% \centering
% \begin{tabular}{p{0.6\linewidth}p{0.2\linewidth}p{0.2\linewidth}}
%     \hline
%     \textbf{Query}  \\
%     \textbf{Before training:} [book_flight(access_token='abc123xyz', card_id='card_123456789', travel_date='2024-04-15', travel_from='LAX', travel_to='JFK', travel_class='business', travel_cost=1000.0)] \\
%     \textbf{Response:} \textcolor{blue}{Based on the provided passages, Republicans use a proportional method to allocate delegates in their presidential nominating procedure.} [\texttt{SynCheck: 0.849}] \textcolor{blue}{According to passage 1, some states award delegates to candidates on a winner-take-all basis, while others award delegates in proportion to each candidate's share of the primary vote.} [\texttt{SynCheck: 0.964}] \textcolor{red}{This suggests that the allocation of delegates is not solely determined by a simple majority vote, but rather takes into account the distribution of support among the various candidates.} [\texttt{SynCheck: 0.302}] \textcolor{red}{Therefore, the answer to the question is: Proportional.} [\texttt{SynCheck: 0.827}] \\
%     \hline     
%     \textbf{Instruction:} Summarize the following news within 53 words \\
%     \textbf{Context:} Their relationship led to jail time for her, but Mary Kay Letourneau Fualaau wants the world to know that she and her husband, Vili Fualaau, are still happily together. She was a married 34-year-old teacher and mother of four in Seattle in 1996 when she began an affair with Fualaau, her 13-year-old student. Letourneau gave birth to her young lover's child and went on to serve more than seven years in prison on charges related to their sexual relationship. On Friday, ABC's "20/20" will air an exclusive interview with the couple, who will celebrate their 10th wedding anniversary on May 20. The pair wed soon after she was released from prison in 2005 and are now the parents of two teen girls. According to ABC, during the interview with Barbara Walters, "Mary Kay tells Walters what makes their marriage work in spite of their huge difference in their age." "She also discusses her surprising plans to teach again, as well as her intentions to have her status as a registered sex offender lifted," a posting on the network's site says. "Vili Fualaau, meanwhile, discusses his bouts with alcoholism, depression and why he believes the system failed him while he was still a minor." Letourneau Fualaau is now 53, and her husband is 31.\\
%     \textbf{Response:} \textcolor{blue}{Mary Kay Letourneau, who served 7 years in prison for having an affair with her 13-year-old student, is still married to her husband Vili Fualaau and they are celebrating their 10th wedding anniversary this May.} [\texttt{SynCheck: 0.974}] \textcolor{red}{Despite their large age gap, they claim their marriage works due to their shared values and love for each other.} [\texttt{SynCheck: 0.627}] \textcolor{blue}{Letourneau hopes to become a teacher again and has applied to have her sex offender status lifted.} [\texttt{SynCheck: 0.945}] \\
%     \hline 
%     \textbf{Instruction:} Write an objective overview about the following local business based only on the provided structured data. \\
%     \textbf{Context:} \{'name': 'Super Cucas', 'address': '6527 Madrid Rd', 'city': 'Isla Vista', 'state': 'CA', 'categories': 'Ethnic Food, Specialty Food, Local Flavor, Mexican, Restaurants, Food, Breakfast \& Brunch, Fast Food, Juice Bars \& Smoothies', 'hours': \{'Monday': '7:0-0:0', 'Tuesday': '7:0-0:0', 'Wednesday': '7:0-0:0', 'Thursday': '7:0-0:0', 'Friday': '7:0-0:0', 'Saturday': '7:0-0:0', 'Sunday': '7:0-0:0'\}, 'attributes': \{'BusinessParking': \{'garage': False, 'street': True, 'validated': False, 'lot': None, 'valet': False\}, 'RestaurantsReservations': False, 'OutdoorSeating': None, 'WiFi': 'no', 'RestaurantsTakeOut': True, 'RestaurantsGoodForGroups': True, 'Music': None, 'Ambience': \{'touristy': False, 'hipster': False, 'romantic': False, 'divey': None, 'intimate': False, 'trendy': False, 'upscale': False, 'classy': False, 'casual': True\}\}, 'business\_stars': 3.5, 'review\_info': [\{'review\_stars': 4.0, 'review\_date': '2021-11-03 21:59:35', 'review\_text': "Super Cucas is really tasty and the portion sizes are so generous. They're also open late which is always great when you're in a college town. I love that they have a menu that offers every style of meat veganized (including soy pastor!) I'd love to try the vegan fries with meat (asada fries) and the breakfast burritos on my next visit. The portions are huge so I would recommend splitting or saving for 2 meals."\}]\}\\
%     \textbf{Response:} \textcolor{blue}{Super Cucas is a locally-owned restaurant located in Isla Vista, California, serving a variety of Ethnic, Specialty, and Mexican cuisine.} [\texttt{SynCheck: 0.939}] \textcolor{red}{With a rating of 3.5 stars, the restaurant is popular among locals and visitors alike, particularly for its late hours of operation (until 10 PM from Monday to Saturday).} [\texttt{SynCheck: 0.594}] \textcolor{blue}{The establishment is known for its generous portion sizes and vegetarian options, including veganized meats.} [\texttt{SynCheck: 0.988}] \textcolor{blue}{While some reviewers have praised the quality of the food, others have experienced poor customer service, with instances of incorrect orders and rude staff behavior.} [\texttt{SynCheck: 0.801}] \textcolor{red}{Nonetheless, Super Cucas remains a popular spot for those seeking tasty and affordable meals in the area.} [\texttt{SynCheck: 0.794}]
%     \\
%     \hline
% \end{tabular}
% \caption{Examples of fixing different types of errors in multi-turn challenges after training on our synthesized data.}
% \label{qualitative-study-selection}
% \end{figure*}

